RoSE-Opt: Robust and Efficient Analog Circuit Parameter Optimization with Knowledge-infused Reinforcement Learning

This paper proposes a learning framework, RoSE-Opt, to achieve robust and efficient analog circuit parameter optimization. RoSE-Opt has two important features. First, it incorporates key domain knowledge of analog circuit design, such as circuit topology, couplings between circuit specifications, and variations of process, supply voltage, and temperature, into the learning loop. This strategy facilitates the training of an artificial agent capable of achieving design goals by identifying device parameters that are optimal and robust. Second, it exploits a two-level optimization method, that is, integrating Bayesian optimization (BO) with reinforcement learning (RL) to improve sample efficiency. In particular, BO is used for a coarse yet quick search of an initial starting point for optimization. This sets a solid foundation to efficiently train the RL agent with fewer samples. Experimental evaluations on benchmarking circuits show promising sample efficiency, extraordinary figure-of-merit in terms of design efficiency and design success rate, and Pareto optimality in circuit performance of our framework, compared to previous methods. Furthermore, this work thoroughly studies the performance of different RL optimization algorithms, such as Deep Deterministic Policy Gradients (DDPG) with an off-policy learning mechanism and Proximal Policy Optimization (PPO) with an on-policy learning mechanism. This investigation provides users with guidance on choosing the appropriate RL algorithms to optimize the device parameters of analog circuits. Finally, our study also demonstrates RoSE-Opt's promise in parasitic-aware device optimization for analog circuits. In summary, our work reports a knowledge-infused BO-RL design automation framework for reliable and efficient optimization of analog circuits' device parameters.

==> ppo_algorithm.tex <==
\begin{algorithm}[!t]
\caption{PPO-Clip}
\begin{footnotesize}
\begin{algorithmic}[1]

\State Input: initial policy parameters $\theta_0$, inital value function parameters $\phi_0$
\For{$k=0,1,2,\cdots$}
    
    \State Collect set of trajectories $\mathcal{D}_k=\{\tau_i\}$ by running policy $\pi_k=\theta_k$ in the circuit design environment.
    \State Compute rewards-to-go $\hat{R}_t$ for the trajectories/episodes.
    \State Compute advantage estimates, $\hat{A}_t$ (using any method of advantage estimation) based on the current value function $V_{\phi_k}$.
    \State Update the policy by maximizing the PPO-clip objective in Eq.~\eqref{eq:ppo}, typically via stochastic gradient ascent with Adam~\cite{adam}.
    \State Fit value function by regression on mean-squared error:
    \begin{equation}
 \phi_{k+1}= \arg \min\dfrac{1}{|\mathcal{D}_k|T}\sum_{\tau\in\mathcal{D}_k}\sum_{t=0}^T(V_{\phi}(s_t)-\hat{R}_t)^2,\nonumber 
\label{eq:ppo_va}
\end{equation}
    typically via stochastic gradient ascent with Adam~\cite{adam}.
\EndFor

\State \textbf{end for}
\end{algorithmic}
\label{alg: ppo}
\end{footnotesize}
\end{algorithm}

==> tab_device_para_2.tex <==
\begin{table*}[!t]
%\vskip -0.15in
\caption{Design space of device parameters and sampling space of desired specifications of two benchmarks.}
%\vskip 0.05in
\begin{center}
\begin{footnotesize}
\vskip -0.1in
\begin{tabular}{c|cccc|cc}
\toprule
Circuit types                                                       & \multicolumn{4}{c|}{Two-stage Op-Amp} & \multicolumn{2}{c}{RF PA} \\ 
\midrule
Implementation technology & \multicolumn{4}{c|}{45 nm CMOS}       & \multicolumn{2}{c}{150 nm GaN}           \\ \hline
\# of device parameters  & \multicolumn{4}{c|}{$2\cdot7 + 1 =15$}      & \multicolumn{2}{c}{$2\cdot7=14$}               \\ \hline
\begin{tabular}[c]{@{}c@{}}Parameter \\ constraints\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Width ($\mu$m)\\ $[1,100]$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\# of fingers\\ $[2, 32]$\end{tabular} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}capacitance (\textit{p}F)\\ $[0.1, 10]$\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Width ($\mu$m)\\ $[16,100]$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\# of fingers\\ $1, 2,4,...,16$\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Desired specifications\\ ( Sampling space)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Gain ($G$)\\ $[300, 500]$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Bandwidth ($B$)\\ $[10^6, 2.5\cdot 10^7]$ Hz\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Phase\\  margin ($PM$)\\ $[55^{\circ}, 60^{\circ}]$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Power \\ consumption ($P$)\\ $[10^{-4}, 10^{-2}]$ W\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Power \\ efficiency ($E$)\\ $[50\%, 60\%]$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Output \\ power ($P$)\\ $[2,3]$ W\end{tabular} \\   \bottomrule
\end{tabular}
\end{footnotesize}
\end{center}
\label{tab1}
%\vskip -0.1in
\end{table*}

==> table_com_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[!htb]
% \caption{Comparison of different methods in searching optimal device parameters for the given specifications.}
% \begin{center}
% \begin{small}
% %\begin{sc}
% \vskip 3pt
% \begin{tabular}{cccc}
% %\toprule
% \hline
% \multirow{2}{*}{Methods} &
%   \multicolumn{2}{c|}{Mean \# of iterations} &
%   \multirow{2}{*}Generality\\ \cline{2-3}
%  &
%   \begin{tabular}[c]{@{}c@{}}Two-stage\\ Op-Amp\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}RF \\ polar-TX\end{tabular} &
%   \\ \hline
% \begin{tabular}[c]{@{}c@{}}Bayesian \\ optimization\\\cite{bayesian}\end{tabular}      &50  &50  & $\times$   \\ \hline
% \begin{tabular}[c]{@{}c@{}}FCNN-based\\ policy network\\\cite{autockt_berke} \end{tabular}   &25  &22  & $\times$ \\ \hline
% \begin{tabular}[c]{@{}c@{}}GCN-FC-based\\ policy network\end{tabular} &20  & 17 &$\surd$ \\ \hline
% \end{tabular}
% %\end{sc}
% \end{small}
% \end{center}
% \label{tab2}
% \end{table}

\iffalse

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\caption{Comparison of different methods in searching optimal device parameters for the given specifications.}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{Methods} &
  \multicolumn{2}{c}{Mean \# of steps} &
  \multirow{2}{*}{Generality} \\ \cline{2-3}
 &
  \begin{tabular}[c]{@{}c@{}}Two-stage\\ Op-Amp\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RF\\ polar-TX\end{tabular} &
   \\ 
   %\hline
\midrule
\begin{tabular}[c]{@{}c@{}}Bayesian \\ optimization\end{tabular}      &50  &50  &$\times$   \\ %\hline
\\
\begin{tabular}[c]{@{}c@{}}FCNN-based\\ policy network\end{tabular}   & 25 & 22 & $\times$  \\ %\hline
\\
\begin{tabular}[c]{@{}c@{}}GCN-FC-based\\ policy network\end{tabular} & 20 & 17 & $\surd$ \\ %\hline
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\label{tab2}
\vskip -0.1in
\end{table}
\fi


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
%\vskip -0.1in
\caption{Comparison of different design automation methods.
%in searching optimal device parameters for the given specifications.
}
%\vskip -0.5in
\begin{center}
\begin{small}
%\begin{sc}
\vskip -0.1in
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Methods}} &
  \multicolumn{2}{c|}{Mean \# of design steps} &
  \multirow{2}{*}{Generality} \\ \cline{2-3}
\multicolumn{1}{c|}{} &
  \begin{tabular}[c]{@{}c@{}}Two-stage\\ Op-Amp\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}RF\\ polar-TX\end{tabular}} &
   \\
   \midrule
\begin{tabular}[c]{@{}c@{}}Bayesian\\ Optimization\\\cite{bayesian}\end{tabular}       & 105 & 86 & $\times$  \\\hline
\begin{tabular}[c]{@{}c@{}}FCNN-based\\ policy network\\\cite{autockt_berke}\end{tabular}   & 25 & 22 & $\times$  \\\hline
\begin{tabular}[c]{@{}c@{}}GNN-FC-based\\ policy network\end{tabular} & 20 & 17 & $\surd$ \\ \bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\label{tab2}
%\vskip -0.10in
\end{table}

==> table_confi.tex <==

\iffalse
\begin{table*}[!hbt]
%\vskip -0.1in
\caption{Training configurations by using the design of two-stage Op-Amps as an example.}
\begin{center}
\begin{small}
\vskip -0.1in
\begin{tabular}{c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{Policies} &
  \begin{tabular}[c]{@{}c@{}}GNN-FC-based\\  policy network\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}GCN-based \\ policy network\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}FCNN-based\\  policy network\end{tabular} \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Policy network\\ parameters\end{tabular}} &
  Architecture &
  GCN (GAT) + FC &
  GCN &
  FCNN \\ \cline{2-5} 
 &
  Network parameter &
  \begin{tabular}[c]{@{}c@{}}GCN: ${[}64, 64, 4{]}$; FCNN:${[}32, 32, 45{]}$ \\GAT: ${[}64, 64, 4{]}$; FCNN:${[}32, 32, 45{]}$; heads: 3\end{tabular} & ${[}64, 64, 45{]}$
   & ${[}64, 64, 45{]}$
   \\ \hline
\begin{tabular}[c]{@{}c@{}}Optimizer\\ parameters\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Optimizer\\ Learning rate\\ $\beta$\\ $\gamma$\end{tabular} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Adam~\cite{adam}\\ 0.0005\\ {[}0.9, 0.9{]}\\ 0.95\end{tabular}} \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}PPO~\cite{ppo}\\ parameter\end{tabular}} &
  Clip parameter &
  \multicolumn{3}{c}{0.3} \\ \cline{2-5} 
 &
  \begin{tabular}[c]{@{}c@{}}Epochs for\\  policy updating\end{tabular} &
  \multicolumn{3}{c}{10} \\ \cline{2-5} 
 &
  Training episodes &
  \multicolumn{3}{c}{35000} \\ \cline{2-5} 
 &
  \begin{tabular}[c]{@{}c@{}}Episodes for policy\\ parameter updating\end{tabular} &
  \multicolumn{3}{c}{30} \\ \cline{2-5} 
 &
  Episode steps &
  \multicolumn{3}{c}{50} \\  \bottomrule
\end{tabular}
\end{small}
\end{center}
\label{tab_con}
%\vskip -0.1in
\end{table*}
\fi






\begin{table*}[!t]
\caption{Training configurations by using the design of two-stage Op-Amps as an example.}
\begin{center}
\begin{footnotesize}
\vskip -0.10in
\begin{tabular}{c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{RL methods} &
Our RL method&
 RL method (Baseline B)  \cite{GCN_RL_MIT} &
  RL method (Baseline A)  \cite{autockt_berke, RL_1} \\ \midrule
\multirow{3}{*}{Policy network} &
  Architecture &
  GCN (GAT) + FC &
  GCN (GAT) &
  FCNN \\ \cline{2-5} 
 &
  Network parameter &
  \begin{tabular}[c]{@{}c@{}}GCN: ${[}64, 64, 4{]}\times 3$; FCNN:${[}32, 32, 45{]}$ \\GAT: ${[}64, 64, 4{]}$; FCNN:${[}32, 32, 45{]}$; heads: 3\end{tabular} & Our GCN (GAT) part
  &  ${[}64, 64, 4{]}\times 3 + {[}32, 32, 45{]}$ % ${[}{[}64, 64, 4{]}\times 3 + {[}32, 32, 45{]}{]}$
  \\ \hline
\begin{tabular}[c]{@{}c@{}}Optimizer\\ parameters\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Optimizer\\ Learning rate\\ $\beta$\\ $\gamma$\end{tabular} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Adam~\cite{adam}\\ 0.0005\\ {[}0.9, 0.9{]}\\ 0.95\end{tabular}} \\ \hline
\multirow{7}{*}{PPO parameter~ \cite{ppo}} &
  Clip parameter &
  \multicolumn{3}{c}{0.3} \\ \cline{2-5} 
 &
  \begin{tabular}[c]{@{}c@{}}Epochs for\\  policy updating\end{tabular} &
  \multicolumn{3}{c}{10} \\ \cline{2-5} 
 &
  Training episodes &
  \multicolumn{3}{c}{35000} \\ \cline{2-5} 
 &
  \begin{tabular}[c]{@{}c@{}}Episodes for policy\\ parameter updating\end{tabular} &
  \multicolumn{3}{c}{30} \\ \cline{2-5} 
 &
  Episode steps &
  \multicolumn{3}{c}{50} \\  \bottomrule
\end{tabular}
\end{footnotesize}
\end{center}
\label{tab_con}
\end{table*}




==> table_sum.tex <==


\begin{table*}[!t]
%\vskip -0.5in
\caption{Comparison summarization of different design automation methods.}
\begin{center}
\begin{footnotesize}%scriptsize
\vskip -0.15in
\begin{threeparttable}
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\multirow{3}{*}{Methods} &
   \multicolumn{2}{c|}{\multirow{3}{*}{Key domain knowledge (YES or NO)}} &
  \multicolumn{3}{c|}{P2S optimization} &
  FoM optimization \\ \cline{4-7} 
 &
  \multicolumn{2}{c|}{} &
  %\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Design\\ accuracy\end{tabular}} 
  \multirow{2}{*}{Design accuracy}&
  \multicolumn{2}{c|}{Mean \# of design steps} &
  FoM value \\ \cline{5-7} 
 &
  \multicolumn{2}{c|}{} &
   &
  Two-stage Op-Amp &
  RF PA &
  RF PA \\ \midrule
Genetic Algorithm~\cite{genetic} &
  \multicolumn{2}{c|}{NO} & 76.7\%
   & 370
   & 389
   & 2.53
   \\ \hline
Bayesian Optimization~\cite{bayesian} &
  \multicolumn{2}{c|}{NO} & 83.7\%
   & 86
   & 105
   & 2.61
   \\ \hline
Supervised learning~\cite{op_amp_FCNN} &
  \multicolumn{2}{c|}{NO} & 79\%
   & 1
   & 1
   & N/A
   \\ \hline
RL method (Baseline A)~\cite{autockt_berke} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}NO
  %: Device parameters, intermediate specifications,\\  and desired specifications as states
  \end{tabular}} & 92\%
   & 27
   & 23\tnote {a}
   & 2.92\tnote {a}
   \\ \hline
RL method (Baseline B)~\cite{GCN_RL_MIT} &  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}NO\tnote {b}\end{tabular}}
   & 84\% (87\%)
   & 32 (31)
   & 25 (23)\tnote {a}
   & 2.81 (2.86)\tnote {a}
   \\ \hline
\multirow{2}{*}{\textbf{Our RL method}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{YES: %Full circuit topology}  + \\ \textbf{Coupling of circuit specifications
  }\end{tabular}} & 
  \textbf{GCN + FCNN} & \textbf{98\%}
   & \textbf{24}
   & \textbf{19}
   & \textbf{3.18}
   \\ \cline{3-7} 
 &
   &
 \textbf{ GAT + FCNN} &\textbf{99\%}
   & \textbf{21}
   & \textbf{16}
   & \textbf{3.25}
   \\   \bottomrule
\end{tabular}
\begin{tablenotes}\scriptsize
\item[a] They originally could not design RF circuits. We use our transfer-learning technique to enable them to design RF circuits.
\item[b] Implemented with our GCN (GAT) part: full circuit topology $+$ device parameters as key node features.
\end{tablenotes}
\end{threeparttable}
\end{footnotesize}%scriptsize
\label{tab2}
\end{center}
\vskip -12pt
\end{table*}
